Reduced Order Internal Models in the Frequency Domain

The internal model principle states that all robustly regulating controllers must contain a suitably reduplicated internal model of the signal to be regulated. Using frequency domain methods, we show that the number of the copies may be reduced if the class of perturbations in the problem is restricted. We present a two stage design procedure for a simple controller containing a reduced order internal model achieving robust regulation. The results are illustrated with an example of a five tank laboratory process where a restricted class of perturbations arises naturally.

==> CustomCommands.tex <==
%\ProvidesPackage{CustomCommands}

\usepackage{ifthen}
\newcommand*{\keyterm}[1]{\emph{#1}}% Math Operators
\DeclareMathOperator{\re}{Re}			% Real Part
\DeclareMathOperator{\im}{Im}			% Imaginary Part
\DeclareMathOperator*{\Res}{Res}		% Residue
\DeclareMathOperator{\rank}{rank}		% Rank
\DeclareMathOperator{\diag}{diag}		% Diagonal
\DeclareMathOperator{\Tr}{Tr}			% Trace
\DeclareMathOperator{\adj}{adj}		% Classical Adjoint
\DeclareMathOperator{\spr}{spr}		% Spectral Radius
\DeclareMathOperator{\Span}{span}		% Span
\DeclareMathOperator{\Gr}{Gr}			% Graph of a mapping
\DeclareMathOperator*{\lcm}{lcm}         % Least Common Multiple
\DeclareMathOperator{\supp}{supp}        % Support
%\DeclareMathOperator{\ran}{ran}          % Range
\newcommand{\ran}{\mathcal{R}}						% Range
\renewcommand{\ker}{\mathcal{N}}					% Null space
\DeclareMathOperator*{\essup}{ess\,sup}  % Essential Supremum
\DeclareMathOperator*{\vrai}{vrai}
\DeclareMathOperator*{\wlim}{w-lim}      % Weak Limit
\DeclareMathOperator*{\slim}{s-lim}      % Strong Limit
\DeclareMathOperator*{\ulim}{u-lim}      % Uniform Limit
\DeclareMathOperator*{\dist}{dist}       % Distance between sets
\DeclareMathOperator*{\diam}{diam}       % Diameter of a set
\DeclareMathOperator*{\card}{card}       % Cardinality of a set
\DeclareMathOperator{\codim}{codim}			 % Co-dimension
\DeclareMathOperator{\alg}{alg}					% Algebraic multiplicity
\DeclareMathOperator{\geom}{geom}					% Geometric multiplicity
\DeclareMathOperator{\sinc}{sinc}
%\DeclareMathOperator{\Arg}{Arg} 	% Principal argument

% Elementary functions
% Names starting with capital letters are principal branches.
\DeclareMathOperator{\Arg}{Arg}
\DeclareMathOperator{\Log}{Log}
\DeclareMathOperator{\Ln}{Ln}
\DeclareMathOperator{\arccot}{arccot}
\DeclareMathOperator{\Arcsin}{Arcsin}
\DeclareMathOperator{\Arccos}{Arccos}
\DeclareMathOperator{\Arctan}{Arctan}
\DeclareMathOperator{\Arccot}{Arccot}
\DeclareMathOperator{\arcsinh}{arcsinh}
\DeclareMathOperator{\arccosh}{arccosh}
\DeclareMathOperator{\arctanh}{arctanh}
\DeclareMathOperator{\arccoth}{arccoth}
\DeclareMathOperator{\Arcsinh}{Arcsinh}
\DeclareMathOperator{\Arccosh}{Arccosh}
\DeclareMathOperator{\Arctanh}{Arctanh}
\DeclareMathOperator{\Arccoth}{Arccoth}

\DeclareMathOperator{\sign}{sign}

% Direct and orthogonal sums
\newcommand{\dirsum}{\oplus}
\newcommand{\orthsum}{\oplus_{\hspace{-1pt}\raisebox{-1pt}{\mbox{\scriptsize$\bm{\perp}$}}\hspace{-2pt}}}


% Variable size delimiters.
% The first argument is the size: big, bigg, etc.
% The second argument is the delimiter: \{, [, (, etc.
\newcommand*{\ldelim}[2]{\csname#1l\endcsname#2}   % Left
\newcommand*{\rdelim}[2]{\csname#1r\endcsname#2}   % Right
\newcommand*{\mdelim}[2]{\csname#1m\endcsname#2}   % Middle

% Horizontal space the amount of a relational symbol
\newcommand*{\relspace}[1][=]{\mathrel{\phantom{#1}}}
% Raise a superscript
\newcommand*{\raisesp}[2]{\raisebox{#1}{\mbox{$\scriptstyle#2$}}}

% Greek letters
\newcommand{\ga}{\alpha}
\newcommand{\gb}{\beta}
\newcommand{\gc}{\chi}
\renewcommand{\gg}{\gamma}
\newcommand{\gd}{\delta}
\newcommand{\gf}{\varphi}
\newcommand{\gl}{\lambda}
\newcommand{\gw}{\omega}
\newcommand{\gs}{\sigma}
\newcommand{\gt}{\tau}
\newcommand{\gz}{\zeta}
\newcommand{\eps}{\varepsilon}

% Symbols
\newcommand*{\C}{{\mathbb{C}}}     % Complex
\newcommand*{\Cp}{{\mathbb{C}^+}}
\newcommand*{\R}{{\mathbb{R}}}     % Real
\newcommand*{\Q}{{\mathbb{Q}}}     % Rational
\newcommand*{\Z}{{\mathbb{Z}}}     % Integer
\newcommand*{\N}{{\mathbb{N}}}     % Natural

% Upright letters

\newcommand*{\me}{{\mathrm{e}}}
\newcommand*{\mi}{{\mathrm{i}}}
\newcommand*{\md}{{\mathrm{d}}}
\newcommand*{\mD}{{\mathrm{D}}}
\newcommand*{\minsv}{\sigma_{\textnormal{min}}}   % Minimum singular value
\newcommand*{\maxsv}{\sigma_{\textnormal{max}}}   % Maximum singular value
\newcommand*{\Lin}{{\mathcal{L}}}   % Bounded Linear Operators
\newcommand*{\Clo}{\mathcal{C}}     % Closed Linear Operators
\newcommand*{\Comp}{\mathcal{K}}		% Compact Linear Operators
\newcommand*{\Dom}{{\mathcal{D}}}   % Domain
\newcommand*{\Ran}{{\mathcal{R}}}   % Range
\newcommand*{\Nul}{{\mathcal{N}}}   % Nullspace
\newcommand*{\Contr}{{\mathcal{B}}} % Controllability map
\newcommand*{\Obser}{{\mathcal{C}}} % Observability map

% Fixed size absolute value etc.
\newcommand*{\abs} [1]{\lvert#1\rvert}
\newcommand*{\norm}[1]{\lVert#1\rVert}
\newcommand*{\seminorm}[1]{\abs{#1}}
\newcommand*{\set} [1]{\{#1\}}
\newcommand*{\setm}[2]{\{\,#1\mid#2\,\}}   % Set with middle |
\newcommand*{\iprod}[2]{\langle#1,#2\rangle}    % Inner Product
\newcommand*{\dualpair}[2]{\langle#1,#2\rangle}
\newcommand*{\pair}[2]{\left(#1,#2\right)} % Ordered pair
\newcommand*{\conv}[2]{#1\ast#2}
\newcommand*{\seq}[2]{(#1)_{#2}^\infty}  % Sequence
\newcommand*{\seqn}[2][]{(#2)_{#1}}      % Sequence
\newcommand*{\ceil} [1]{\lceil#1\rceil}
\newcommand*{\floor}[1]{\lfloor#1\rfloor}
\newcommand*{\bin}[2]{\left(\mat{#1\\#2}\right)}

% Variable size absolute value etc.
% The optional first argument is the size: big, bigg, etc.
% The default is to use automatic sizing with \left and \right.
\newcommand*{\Abs}[2][default]{\ifthenelse{\equal{#1}{default}}{\left\lvert#2\right\rvert}{\ldelim{#1}{\lvert}#2\rdelim{#1}{\rvert}}}
\newcommand*{\Norm}[2][default]{\ifthenelse{\equal{#1}{default}}{\left\lVert#2\right\rVert}{\ldelim{#1}{\lVert}#2\rdelim{#1}{\rVert}}}
\newcommand*{\Seminorm}[2][default]{\Abs[#1]{#2}}
\newcommand*{\Iprod}[3][default]{\ifthenelse{\equal{#1}{default}}{\left\langle#2,#3\right\rangle}{\ldelim{#1}{\langle}#2,#3\rdelim{#1}{\rangle}}}
\newcommand*{\Dualpair}[3][default]{\ifthenelse{\equal{#1}{default}}{\left\langle#2,#3\right\rangle}{\ldelim{#1}{\langle}#2,#3\rdelim{#1}{\rangle}}}
\newcommand*{\Seq}[2]{\left(#1\right)_{#2}^\infty}
\newcommand*{\Seqn}[2][]{\left(#2\right)_{#1}}
\newcommand*{\List}[2][1]{\set{#1,\ldots,#2}}

% Set
% Variable size braces.
% The optional first argument is the size: big, bigg, etc.% The default is to use automatic sizing with \left and \right.
\newcommand*{\Set}[2][default]{\ifthenelse{\equal{#1}{default}}{\left\{#2\right\}}{\ldelim{#1}{\{}#2\rdelim{#1}{\}}}}

% Set with middle
% Variable size braces and |.
% The optional first argument is the size: big, bigg, etc.
% The default is big.
\newcommand*{\Setm}[3][big]{\ldelim{#1}{\{}\,#2\mdelim{#1}{|}#3\,\rdelim{#1}{\}}}

% Partial Derivative
%\newcommand*{\dd}[1][x]{\frac{d}{d#1}}
\newcommand*{\dda}[3][1]{\ifthenelse{\equal{#1}{1}}{\frac{d#3}{d#2}}{\frac{d^{#1}#3}{d#2^{#1}}}}
\newcommand*{\ddb}[2][1]{\ifthenelse{\equal{#1}{1}}{\frac{d}{d#2}}{\frac{d^{#1}}{d#2^{#1}}}}
\newcommand*{\pd}[3][1]{\ifthenelse{\equal{#1}{1}}{\frac{\partial{#2}}{\partial{#3}}}{\frac{\partial^{#1}{#2}}{\partial#3^{#1}}}}
\newcommand*{\pdb}[2][1]{\ifthenelse{\equal{#1}{1}}{\frac{\partial}{\partial{#2}}}{\frac{\partial^{#1}}{\partial#2^{#1}}}}
\newcommand*{\pdd}[3]{\frac{\partial^2{#1}}{\partial{#2}\partial{#3}}}
% Substitution (in integral)
\newcommand{\subst}{\bigg\lvert}
% Matrix
\newcommand{\Matrix}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\Det}[1]{\begin{vmatrix}#1\end{vmatrix}}
\newcommand{\Array}[2]{\left[\begin{array}{#1}#2\end{array}\right]}

% Complex Conjugate, Closure, Boundary, Complement
\newcommand*{\conj}[1]{\overline{#1}}
\newcommand*{\closure}[1]{\overline{#1}}
\newcommand{\boundary}{\partial}
\newcommand*{\Complement}{\mathord{\thicksim}}

% Limits from the left and right
\newcommand{\lto}{\uparrow}
\newcommand{\rto}{\downarrow}
\newcommand*{\limn}[1][n]{\lim_{#1\to\infty}}

% Arrows (abbreviations)
%\newcommand{\to}{\rightarrow}
\newcommand{\from}{\leftarrow}
\newcommand{\too}{\longrightarrow}
\newcommand{\tofrom}{\leftrightarrow}
\newcommand{\froom}{\longleftarrow}
\newcommand{\To}{\Rightarrow}
\newcommand{\From}{\Leftarrow}

% Algebra
\newcommand*{\semigroup}[1]{\mathcal{#1}}
\newcommand*{\monoid}[1]{\mathcal{#1}}
\newcommand*{\group}[1]{\mathcal{#1}}
\newcommand*{\ring}[1]{\mathcal{#1}}
\newcommand*{\field}[1]{\mathbb{#1}}
\newcommand*{\divides} [2]{{#1}|{#2}}
\newcommand*{\rdivides}[2]{{#1}|_R\,{#2}}
\newcommand*{\ldivides}[2]{{#1}|_L\,{#2}}

% Misc
\newcommand*{\Xloc}[1]{#1_{\text{loc}}}
\newcommand*{\Lploc}[1][p]{\Xloc{L^{#1}}}
\newcommand*{\Lp}[1][p]{L^{#1}}
\newcommand*{\lp}[1][p]{\ell^{#1}}
\newcommand*{\half}[1][2]{\frac{1}{#1}}
\newcommand*{\range}[3][i]{{#2}\le{#1}\le{#3}}
\newcommand*{\cartesian}{\text{\Large $\times$}}
\newcommand*{\inverse}{^{-1}}
\newcommand*{\inv}{^{-1}}

%\renewcommand{\vec}[1]{\mathbf{#1}}
\renewcommand{\vec}[1]{\underline{#1}}

% Referencing Sections, Theorems etc.
\newcommand*{\refCh}[1]{Chapter~\ref{#1}}        % Chapter
\newcommand*{\refch}[1]{chapter~\ref{#1}}        % lower case
\newcommand*{\refSec}[1]{Section~\ref{#1}}       % Section
\newcommand*{\refsec}[1]{section~\ref{#1}}       % 
\newcommand*{\refFig}[1]{Figure~\ref{#1}}        % Figure
\newcommand*{\reffig}[1]{figure~\ref{#1}}        % 
\newcommand*{\refTbl}[1]{Table~\ref{#1}}         % Table
\newcommand*{\refThm}[1]{Theorem~\ref{#1}}       % Theorem
\newcommand*{\refthm}[1]{theorem~\ref{#1}}       % 
\newcommand*{\refPrp}[1]{Proposition~\ref{#1}}   % Proposition
\newcommand*{\refprp}[1]{proposition~\ref{#1}}   % 
\newcommand*{\refLem}[1]{Lemma~\ref{#1}}         % Lemma
\newcommand*{\reflem}[1]{lemma~\ref{#1}}         % 
\newcommand*{\refCor}[1]{Corollary~\ref{#1}}     % Corollary
\newcommand*{\refcor}[1]{corollary~\ref{#1}}     % 
\newcommand*{\refDef}[1]{Definition~\ref{#1}}    % Definition
\newcommand*{\refdef}[1]{definition~\ref{#1}}    % 
\newcommand*{\refRem}[1]{Remark~\ref{#1}}	 % Remark			 % Remark
\newcommand*{\refrem}[1]{remark~\ref{#1}}	 %			 % 
\newcommand*{\refPro}[1]{Problem~\ref{#1}}       % Problem
\newcommand*{\refExa}[1]{Example~\ref{#1}}       % Example
\newcommand*{\refexa}[1]{example~\ref{#1}}       % 
\newcommand*{\refExe}[1]{Exercise~\ref{#1}}      % Exercise
\newcommand*{\refEq}[1]{Equation~\eqref{#1}}     % Equation
%\newcommand*{\refeq}[1]{equation~\eqref{#1}}     % 
\newcommand*{\refEqs}[1]{Equations~\eqref{#1}}   % Equations
\newcommand*{\refeqs}[1]{equations~\eqref{#1}}   % 
\newcommand*{\refAss}[1]{Assumption~\ref{#1}}    % Assumption
\newcommand*{\refass}[1]{assumption~\ref{#1}}    % 

\DeclareMathOperator*{\AP}{AP}	% Almost periodic functions
\DeclareMathOperator*{\BUC}{BUC}	% BUC functions

\newcommand{\bmat}[1]{\begin{bmatrix}#1\end{bmatrix}}
\newcommand{\bmatsmall}[1]{\begin{bsmallmatrix}#1\end{bsmallmatrix}}
\newcommand{\pmat}[1]{\begin{pmatrix}#1\end{pmatrix}}
\newcommand{\pmatsmall}[1]{\begin{psmallmatrix}#1\end{psmallmatrix}}
\newcommand{\mat}[1]{\begin{matrix}#1\end{matrix}}
\newcommand{\mresult}[1]{\left\{\begin{array}{ll}#1\end{array}\right.}
\newcommand{\mc}[1]{\mathcal{#1}}
\newcommand{\wt}[1]{\widetilde{#1}}
\newcommand{\Csg}{$C_0$-semigroup}
\newcommand{\Cg}{$C_0$-group}


\newcommand{\eq}[1]{\begin{align*}#1\end{align*}}
\newcommand{\eqn}[1]{\begin{align}#1\end{align}}
\newcommand{\ieq}[1]{$#1$}

% Title for notes
\newcommand{\owntitle}[2][\today]{
\clearpage
\begin{center}
{\LARGE #2 \par}
\end{center}
\centerline{\large #1}
}

% Title for notes with author (\owntitleauth[date]{author}{title})
\newcommand{\owntitleauth}[3][\today]{
\clearpage
\begin{center}
{\LARGE #3 \par}
\bigskip
{\large #2}
\end{center}
\centerline{\large #1}
}

% Hide proofs. 
% Usage:
%\newboolean{hideproof}
%\setboolean{hideproof}{true}
%\begin{proof}\hiddenproof{\boolean{hideproof}}{[proof...]}\end{proof}

\newcommand{\hiddenproof}[2]{
\ifthenelse{#1}{Hidden}{#2}
}

\newcommand{\longcomm}[1]{}

\newcommand{\indim}{r}


\usepackage{datetime}
\newdateformat{findate}{\THEDAY.\THEMONTH.\THEYEAR}

\endinput 

